A Rate-Distortion Approach to Caching

This paper takes a rate-distortion approach to understanding the information-theoretic laws governing cache-aided communications systems. Specifically, we characterise the optimal tradeoffs between the delivery rate, cache capacity and reconstruction distortions for a single-user problem and some special cases of a two-user problem. Our analysis considers discrete memoryless sources, expected- and excess-distortion constraints, and separable and f-separable distortion functions. We also establish a strong converse for separable-distortion functions, and we show that lossy versions of common information (G\'{a}cs-K\"{o}rner and Wyner) play an important role in caching. Finally, we illustrate and explicitly evaluate these laws for multivariate Gaussian sources and binary symmetric sources.

==> Figures/two-user-one-cache <==
\begin{figure}[ht!]
\centering
\begin{tikzpicture}[scale=1]
\tikzstyle{every node}=[draw,shape=circle]; 





\path (.5,1.5) node[shape=rectangle,font=\Large] (s0) {$\substack{\text{Library}\\\b{X}_1\ldots,\b{X}_L}$};
\path (2.5,1.5) node[shape=rectangle,minimum height=3.5cm] (s) {$\text{Encoder}$};


\path (6,2) node[shape=rectangle] (d1) {$\text{Decoder} 1$};
\path (6,3) node[shape=rectangle] (c) {$\text{Cache} 1$};

\path (6,0) node[shape=rectangle] (d2) {$\text{Decoder} 2$};

\path (3,3) node[draw=none] (inp1) {};
\path (3,0) node[draw=none] (inp2) {};

\path (8,2) node[draw=none] (s1) {$\hat{\b{X}}_{d_1}$};
\path (8,0) node[draw=none] (s2) {$\tilde{\b{X}}_{d_2}$};




%\draw[->]
  %  (v0) -- (v1) ;
\draw[<->,style=double] (s0) --node[draw=none,yshift=.2cm]{} (s);  


\draw[->] (inp1) --node[draw=none,yshift=.25cm]{$M_c$} (c);
\draw[->] (inp2) --node[draw=none,yshift=-.25cm]{$M_{(d_1,d_2)}$} (d2);
\draw[->] (4.5,0) -| (4.5,2)--(5.2,2);
\draw[->] (d1) -- (s1);
\draw[->] (d2) -- (s2);
\draw[<->,style=double] (c) -- (d1);




\end{tikzpicture}
\caption{Two-user  one-cache RD problem}
\label{two-user-one-cache}
\end{figure}
